Multi-Task Identification of Entities, Relations, and Coreference for Scientific Knowledge Graph Construction

We introduce a multi-task setup of identifying and classifying entities, relations, and coreference clusters in scientific articles. We create SciERC, a dataset that includes annotations for all three tasks and develop a unified framework called Scientific Information Extractor (SciIE) for with shared span representations. The multi-task setup reduces cascading errors between tasks and leverages cross-sentence relations through coreference links. Experiments show that our multi-task model outperforms previous models in scientific information extraction without using any domain-specific features. We further show that the framework supports construction of a scientific knowledge graph, which we use to analyze information in scientific literature.

==> tables/exp_coreference.tex <==
\begin{table}[t]
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\newcommand{\colindent}{\;}
\setlength{\tabcolsep}{.25em}
\footnotesize
\centering
\begin{tabularx}{\linewidth}{l c *{6}{Y}}
\toprule
& \multicolumn{3}{c}{Dev} & \multicolumn{3}{c}{Test} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} 
     Model & P & R & F1 & P & R & F1 \\    
    \midrule
E2E Coref      & 59.4   & 52.0   & 55.4  & 60.9   & 37.3   & 46.2    \\
\sys\ & 61.5   & 54.8   & \textbf{58.0}  & 52.0 & 44.9 & \textbf{48.2} \\
\bottomrule
\end{tabularx}
\caption{Results for coreference resolution. We report average F1 \luheng{cite} for simplicity.}\label{tab:coref}
\end{table}


==> tables/exp_keyphrase_extraction.tex <==
\begin{table}[t]
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\newcommand{\colindent}{\;}
\setlength{\tabcolsep}{.25em}
\footnotesize
\centering
\begin{tabularx}{\linewidth}{l c *{6}{Y}}
\toprule
& \multicolumn{3}{c}{Dev} & \multicolumn{3}{c}{Test} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} 
Model & P & R & F1 & P & R & F1 \\    
\midrule
M\&B \texttt{pipeline}  & 66.7   & 65.9   & 66.3  & 60.8   & 61.2   & 61.0   \\
M\&B \texttt{joint}     & 64.3   & 68.6   & 66.4  & 60.6   & 61.9   & 61.2   \\
M\&B+\texttt{ELMo} & 67.5   & 66.3   & 66.9  & 63.5   & 63.9   & 63.7  \\
%\cmidrule(lr){1-7}
\sys\ & 70.0   & 66.3  & \textbf{68.1}  & 64.4   &  64.7  & \textbf{64.5}  \\
\bottomrule
\end{tabularx}
\caption{Results for scientific keyphrase extraction in terms of labeled precision, recall and F1 on the development and test set. }\label{tab:ner}
\end{table}

==> tables/exp_relation_extraction.tex <==
\begin{table}
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\setlength{\tabcolsep}{.25em}
\footnotesize
\centering
\begin{tabularx}{\columnwidth}{l c *{6}{Y}}
\toprule
& \multicolumn{3}{c}{Dev} & \multicolumn{3}{c}{Test} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} 
Model & P & R & F1 & P & R & F1 \\    
\midrule
M\&B \texttt{pipeline}  & 34.2   & 33.7   & 33.9  & 37.8   & 34.2   & 35.9  \\

M\&B \texttt{joint}    & 37.3   & 33.5   & 35.3  & 37.1   & 32.2   & 34.1  \\
M\&B+\texttt{ELMo} & 38.5   & 36.4   & 37.4  & 38.4   & 34.9   & 36.6  \\
%\cmidrule(lr)
\sys\ & 45.5   & 36.6  & \textbf{40.6}  & 47.9   &  33.8  & \textbf{39.6}  \\
\bottomrule
 \end{tabularx}
\caption{Results for scientific relation extraction in terms of labeled P/R/F1 on development and test set.}\label{tab:relation}
\end{table}

